Review of the semiclassical formalism for multiparticle production at high energies

These notes provide a comprehensive review of the semiclassical approach for calculating multiparticle production rates for initial states with few particles at very high energies. In this work we concentrate on a scalar field theory with a mass gap. Specifically, we look at a weakly-coupled theory in the high-energy limit, where the number of particles in the final state scales with energy, $n\sim E\to \infty$, and the coupling $\lambda\to 0$ with $n \lambda$ held fixed. In this regime, the semiclasical approach allows us to calculate multiparticle rates non-perturbatively.

==> extra_cuts.tex <==
From sec 6.2.1

We make use of the constraint that the energies of the classical solutions 
to the right of the first singular surface on Fig.~\ref{fig:kak_profile}, i.e. for $\tau > \tau_0(\bec{x})$, are known:
\[ 
\tau > \tau_0(\bec{x})\,: \quad E[h_1] \,=\, 0 \,, \qquad  E[h_2]\,=\,nm \:=E >0\,.
\label{eq:Edef12}
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure*}[t]
\begin{center}
\includegraphics[width=0.85\textwidth]{fig_tau1_h12.pdf}
\end{center}
\vskip-.5cm
\caption{Singularity surfaces of the two branches of the solution.
{\bf Plot (a)} depicts the solution branch $h_1(x)$ with the singularity surface at
$\tau_0(\bec{x})$. The energy of this solution vanishes at any value of $\tau$. The integration contour $\int d\tau$ is shown
as the horizontal red arrow with intermediate points $\tau_a$, $\tau_b$ and $\tau_c$.
{\bf Plot (b)} shows $h_2(x)$ with the null surface at $\tau_1(\bec{x})$ annihilating the singularity surface $\tau_0(\bec{x})$.
The remaining singular surface, $\tau_\infty$, is flat. The integration contour $\int d\tau$ is shown
as the horizontal red arrow with intermediate points $\tau_c$, $\tau_d$ and $\tau_e$. The energy of this solution is $E(h_2)=mn$
for $\tau > \tau_\infty$.}
\label{fig:tau1_h12}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The first integral on the right-hand side of \eqref{eq:Se12R22} is over $h_1(x)$: the zero-energy Euclidean-time solution 
in \eqref{clas_sol111Aag}-\eqref{clas_sol222inf}
with the singular surface $\tau_0(\bec{x})$ shown in Fig.~\ref{fig:tau1_h12} (a).
Integration over $\tau$ proceeds from right to left
through the sequence of intermediate values of $\tau$, with three snapshots at  $\tau_a$, $\tau_b$ and $\tau_c$ shown in Fig.~\ref{fig:tau1_h12} (a).
At $\tau=\tau_a$ the Lagrangian and the Euclidean energy of the solution,
\begin{eqnarray}
&&L_{E} \,=\, \int d^3x \left( \frac{1}{2} (\partial_\tau h)^2\,+\, \frac{1}{2} (\partial_{\bec{x}} h)^2\,+\, V(h) \right)\,,
\label{eq:Lhdef}
\\
&&\,\,\,\, E \,=\, \int d^3x \left( -\,\frac{1}{2} (\partial_\tau h)^2\,+\, \frac{1}{2} (\partial_{\bec{x}} h)^2\,+\, V(h) \right)\,,
\label{eq:Ehdef}
\end{eqnarray}
are vanishing. At the lower fixed value $\tau=\tau_b$, the integrals over $d^3x$ 
cross the $\tau_0(\bec{x})$ surface passing between the $h_1=+v$ and the $h_1=-v$ domains. This can be understood as a traversal of the dotted line at $\tau_b$ in Fig.~\ref{fig:tau1_h12} (a).
The Lagrangian density ${\cal L}_{E}$ has a peak at the crossing of $\tau_0(\bec{x})$. As a result, the Lagrangian 
in \eqref{eq:Lhdef} becomes positive at $\tau=\tau_b$, and the action increases from its lower value at $\tau=\tau_a$.
However, the energy of the first solution, $E(h_1)$, must remain vanishing at $\tau_b$, as it is conserved on a classical solution (recall that
there are no infinities of the solution on our shifted contour). 
It is easy to understand why the energy can remain vanishing -- it is the consequence of the negative relative sign
between the kinetic and potential energy density terms in \eqref{eq:Ehdef}. Hence, unlike the expression for the Lagrangian, the energy density 
has positive and negative energy peaks at the crossing that compensate one another on the classical solution.

In summary, the action integral $|\int_{\,+\infty-i\epsilon}^{\,\tau-i\epsilon} d\tau \, L_{E}[h_1]|$ grows with $\tau$ from $\tau=0$
to $\tau=\tau_\infty$ where it crosses the surface $\tau_0(\bec{x})$ separating the $\pm v$ domains of the solution. The action 
on $h_1$ has a non-trivial 
dependence on the shape of $\tau_0(\bec{x})$. Nonetheless, the energy of the solution $h_1$ is vanishing at all values of $\tau$, as required by \eqref{eq:Edef12}. 


************

As we already explained at the start of this subsection, the effect
of the singularity surface at $\tau=\tau_0(\bec{x})$ is cancelled by the null-surface $\tau_1(\bec{x})$.
This is shown in the second plot, Fig.~\ref{fig:tau1_h12} (b). The action integral $\int d\tau \, L_{E}[h_2]$ now starts at 
$\tau_c$ and progresses through the snapshots at $\tau_d$ and $\tau_e$ as indicated in the figure. Only the spatially-flat surface at $\tau_\infty$ is of importance in the calculation of the action and energy. Both action and energy jump by a constant amount
between $\tau<\tau_\infty$ and $\tau<\tau_\infty$. The energy of $h_2$ when $\tau<\tau_\infty$ is $E=mn$. The action integral on $h_2$ is a constant and, importantly, it does not depend on the shape of $\tau_0(\bec{x})$.

